MyMove: Facilitating Older Adults to Collect In-Situ Activity Labels on a Smartwatch with Speech

Current activity tracking technologies are largely trained on younger adults' data, which can lead to solutions that are not well-suited for older adults. To build activity trackers for older adults, it is crucial to collect training data with them. To this end, we examine the feasibility and challenges with older adults in collecting activity labels by leveraging speech. Specifically, we built MyMove, a speech-based smartwatch app to facilitate the in-situ labeling with a low capture burden. We conducted a 7-day deployment study, where 13 older adults collected their activity labels and smartwatch sensor data, while wearing a thigh-worn activity monitor. Participants were highly engaged, capturing 1,224 verbal reports in total. We extracted 1,885 activities with corresponding effort level and timespan, and examined the usefulness of these reports as activity labels. We discuss the implications of our approach and the collected dataset in supporting older adults through personalized activity tracking technologies.

==> tables/demographic_old.tex <==
\begin{table*}[h]

\caption{Summary of demographic of our study participants, their employment status and the latest (or current) occupation, education level, technical proficiency, and IPAQ physical activity category.}
\vspace{-2mm}
    \small\sffamily
    			\def\arraystretch{1.3}
    		    \setlength{\tabcolsep}{0.5em}
    		    \centering
    \begin{tabular}{|l!{\color{lightgray}\vrule}cc!{\color{lightgray}\vrule}ll!{\color{lightgray}\vrule}l!{\color{lightgray}\vrule}l!{\color{lightgray}\vrule}l|}
    \hline
    \rowcolor{tableheader}
    \textbf{ID} & \textbf{Age} & \textbf{Gender} & \multicolumn{2}{!{\color{lightgray}\vrule}l!{\color{lightgray}\vrule}}{\textbf{Employment \& Latest occupation}} & \textbf{Education} & \textbf{Technical proficiency} & \textbf{IPAQ} \\
    \hline
    P1             & 61                               & M            & Retired & Senior manager                           & Bachelor's & Very confident                 & Moderate      \\
    \arrayrulecolor{tablegrayline}\hline
    P2             & 67                               & F          & Self-employed & Visual artist       & Bachelor's & Enjoy the challenge            & Moderate      \\
    \hline
    P3             & 77                               & F          & Retired & Qualitative researcher                            & Ph.D./M.D. & Very confident                 & High          \\
    \hline
    P4             & 70                               & M            & Self-employed & Landlord            & Bachelor's & Enjoy the challenge            & High          \\
    \hline
    P5             & 81                               & F          & Retired & Disability consultant                            & Master's & A little apprehensive          & High          \\
    \hline
    P6             & 79                               & F          & Retired & Policy analyst                             & Master's & Very confident                 & High          \\
    \hline
    P7             & 69                               & F          & Full-time & Business manager        & Master's & Enjoy the challenge            & High          \\
    \hline
    P8             & 90                               & F          & Self-employed & Piano tutor         & Master-level & Enjoy the challenge            & Moderate      \\
    \hline
    P9             & 62                               & F          & Full-time & Communications director  & Master-level  & Very confident                 & Moderate      \\
    \hline
    P10            & 62                               & F          & Retired & Human resource specialist                            & Bachelor's & Very confident                 & Moderate      \\
    \hline
    P11            & 67                               & F          & Retired & Technical training manager                            & Master-level & Enjoy the challenge            & High          \\
    \hline
    P12            & 75                               & F          & Retired & Rehabilitation counselor                            & Master's & Very apprehensive              & High          \\
    \hline
    P13            & 64                               & M            & Retired & Regulatory specialist                            & Master's & Enjoy the challenge            & High   \\
    \arrayrulecolor{black}\hline
    \end{tabular}
\label{table:demographic}
\end{table*}

==> tables/effort-pairwise-comparison.tex <==
\newcommand{\graycell}{\cellcolor[HTML]{e0e0e0}}

\begin{table*}[t]

\caption{Summary of statistical differences showing pairwise
comparisons among 8 effort level categories for each objective physiological metric. Est. represents estimated difference between the two means.  For brevity, only significant pairs are presented.}
\vspace{-2mm}
    \small\sffamily
    			\def\arraystretch{1.4}
    		    \setlength{\tabcolsep}{0.25em}
    		    \centering
\begin{tabular}{|c!{\color{lightgray}\vrule}llp{0.08\textwidth}|lp{0.05\textwidth}C{0.05\textwidth}l|lp{0.05\textwidth}C{0.05\textwidth}l|lp{0.05\textwidth}C{0.05\textwidth}l|}
\hline
\rowcolor{tableheader}           & \multicolumn{3}{l|}{}                    & \multicolumn{4}{l|}{\cellcolor[HTML]{d0d0d0}\textbf{Heart Rate Ratio}}                                      & \multicolumn{4}{l|}{\cellcolor[HTML]{d0d0d0}\textbf{Walking Cadence (activPAL)}}                                        & \multicolumn{4}{l|}{\cellcolor[HTML]{d0d0d0}\textbf{Walking Cadence (Watch)}}                                           \\
\rowcolor{tableheader} \textbf{No.} & \multicolumn{3}{l|}{\textbf{Comparison}} & \multicolumn{2}{l}{Est. (SE)} & $t$-val & $p$-val   & \multicolumn{2}{l}{Est. (SE)} & $t$-val & $p$-val    & \multicolumn{2}{l}{Est. (SE)} & $t$-val & $p$-value    \\
\arrayrulecolor{black}\thicktablehline
\circledigit{1}            & No effort      & vs.     & L-to-M       & 3.95                & (1.06)               & 3.73             & .005**             & 19.28               & (5.06)               & 3.81             & .004**             & \multicolumn{4}{l|}{\graycell}                                                                \\
\arrayrulecolor{tablegrayline}\hline\arrayrulecolor{black}
\circledigit{2}            & No effort      & vs.     & M-to-S       & 5.99                & (1.54)               & 3.90             & .003**             & \multicolumn{4}{l|}{\graycell}                                                                & \multicolumn{4}{l|}{\graycell}                                                                \\
\arrayrulecolor{tablegrayline}\hline\arrayrulecolor{black}
\circledigit{3}            & No effort      & vs.     & Moderate     & 4.31                & (0.80)               & 5.36             & <.001*** & 27.21               & (3.86)               & 7.05             & \textless{}.001*** & 20.57               & (4.19)               & 4.91             & \textless{}.001*** \\
\arrayrulecolor{tablegrayline}\hline\arrayrulecolor{black}
\circledigit{4}            & Low            & vs.     & L-to-M       & \multicolumn{4}{l|}{\graycell}                                                               & 13.13               & (4.12)               & 3.19             & .039*               & \multicolumn{4}{l|}{\graycell}                                                                \\
\arrayrulecolor{tablegrayline}\hline\arrayrulecolor{black}
\circledigit{5}            & Low            & vs.     & M-to-S       & 4.45                & (1.41)               & 3.16             & .036*              & \multicolumn{4}{l|}{\graycell}                                                                & \multicolumn{4}{l|}{\graycell}                                                                \\
\arrayrulecolor{tablegrayline}\hline\arrayrulecolor{black}
\circledigit{6}            & Low            & vs.     & Moderate     & 2.78                & (0.53)               & 5.29             & <.001*** & 21.05               & (2.64)               & 7.98             & \textless{}.001*** & 15.56               & (2.76)               & 5.64             & \textless{}.001*** \\
\arrayrulecolor{tablegrayline}\hline\arrayrulecolor{black}
\circledigit{7}            & Relaxed        & vs.     & Moderate     & \multicolumn{4}{l|}{\graycell}                                                               & 15.91               & (5.07)               & 3.14             & .038*               & \multicolumn{4}{l|}{\graycell}    \\
\hline

\end{tabular}

    \begin{flushleft}
    \hspace{2mm}
    \sffamily\footnotesize{\textbf{***}$p$<.001; \textbf{**}$p$<.01; \textbf{*}$p$<.05}
    \end{flushleft}

\label{table:effort:pairwise}
\end{table*}

==> tables/nlp-experiment.tex <==
\begin{table*}[t]

\caption{$F_{1}$-score, precision, and recall of each activity label averaged over a 10-fold cross validation using a Binary Relevance classifier, with different text sources as a test set. The bottom row summarizes micro-average of the metrics. All numbers are in the unit of \%.}
\vspace{-2mm}
\small\sffamily
    			\def\arraystretch{1.1}
    		    \setlength{\tabcolsep}{0.5em}
    		    \centering
\begin{tabular}{|l|ccc|ccc|ccc|}
\hline
\rowcolor{tableheader}                             & \multicolumn{3}{c|}{\cellcolor[HTML]{d0d0d0}\textbf{Human-transcribed}} & \multicolumn{3}{c|}{\cellcolor[HTML]{d0d0d0}\textbf{Microsoft ASR}} & \multicolumn{3}{c|}{\cellcolor[HTML]{d0d0d0}\textbf{Google ASR}} \\
\arrayrulecolor{darkgray}\cline{2-10}
\rowcolor{tableheader} \textbf{Activity}               & $F_{1}$-score        & Precision     & Recall    & $F_{1}$-score       & Precision   & Recall   & $F_{1}$-score      & Precision  & Recall  \\

\arrayrulecolor{black}\thicktablehline

Caring for pets               & 94.26    & 93.39     & 96.07  & 94.26              & 93.39               & 96.07            & 93.49           & 91.96            & 96.07         \\
Screen time: TV               & 92.63    & 97.12     & 89.33  & 92.63              & 97.12               & 89.33            & 92.31           & 96.36            & 89.33         \\
Screen time: Computer         & 90.09    & 94.36     & 86.54  & 89.24              & 94.90               & 84.71            & 89.37           & 94.33            & 85.37         \\
Reading on paper              & 86.55    & 90.54     & 86.00  & 83.20              & 85.86               & 84.33            & 85.13           & 88.04            & 86.00         \\
Paperwork/desk work           & 85.08    & 96.57     & 77.44  & 83.81              & 96.57               & 76.01            & 85.98           & 96.57            & 78.87         \\
Eating food                   & 81.64    & 92.39     & 73.65  & 80.25              & 92.30               & 71.55            & 79.01           & 90.36            & 70.96         \\
Cleaning/arranging/carrying   & 81.17    & 93.10     & 72.32  & 81.27              & 92.44               & 72.69            & 80.18           & 92.24            & 71.20         \\
Gardening                     & 80.63    & 90.21     & 73.78  & 78.88              & 89.21               & 71.67            & 78.98           & 89.34            & 72.67         \\
Playing puzzle/table game     & 78.33    & 90.00     & 73.33  & 78.33              & 90.00               & 73.33            & 71.67           & 80.00            & 68.33         \\
Seeing at a theater           & 76.67    & 75.00     & 80.00  & 76.67              & 75.00               & 80.00            & 63.33           & 65.00            & 65.00         \\
Driving/in a vehicle          & 75.19    & 87.41     & 68.64  & 74.17              & 86.63               & 67.73            & 75.88           & 88.21            & 68.64         \\
Exercise: Cardio              & 72.57    & 85.66     & 64.24  & 71.20              & 86.37               & 61.59            & 71.03           & 82.17            & 63.41         \\
Personal hygiene              & 72.33    & 90.00     & 63.33  & 72.33              & 90.00               & 63.33            & 75.33           & 90.00            & 66.67         \\
Dressing                      & 71.63    & 88.33     & 66.67  & 65.72              & 77.50               & 60.83            & 71.50           & 85.50            & 65.83         \\
Exercise: Strength/stretching & 70.98    & 93.00     & 59.00  & 74.16              & 93.00               & 63.00            & 69.20           & 93.00            & 57.00         \\
Non-exercise stepping         & 69.62    & 84.24     & 59.64  & 68.23              & 82.66               & 58.46            & 68.76           & 83.59            & 59.05         \\
Preparing food                & 67.12    & 79.43     & 59.49  & 65.32              & 76.27               & 58.65            & 62.91           & 77.96            & 54.49         \\
Napping                       & 64.33    & 73.33     & 63.33  & 59.67              & 61.67               & 60.00            & 73.33           & 85.00            & 68.33         \\
Playing a musical instrument  & 60.00    & 60.00     & 60.00  & 60.00              & 60.00               & 60.00            & 60.00           & 60.00            & 60.00         \\
Screen time: Mobile device    & 58.24    & 72.50     & 53.33  & 49.90              & 67.50               & 43.33            & 47.24           & 57.50            & 43.33         \\
Offline shopping              & 55.17    & 55.50     & 57.50  & 55.17              & 55.50               & 57.50            & 50.67           & 52.50            & 52.50         \\
Crafting/artwork              & 50.00    & 60.00     & 45.00  & 40.00              & 50.00               & 35.00            & 40.00           & 50.00            & 35.00         \\
Voice call                    & 49.78    & 61.67     & 45.83  & 49.78              & 61.67               & 45.83            & 47.02           & 55.83            & 45.83         \\
Nothing/waiting               & 42.98    & 68.50     & 34.33  & 39.71              & 60.50               & 32.33            & 43.40           & 63.17            & 36.33         \\
Face-to-face interaction      & 37.90    & 70.00     & 27.50  & 37.90              & 70.00               & 27.50            & 40.57           & 70.00            & 30.00         \\
Treatment                     & 36.67    & 35.00     & 40.00  & 36.67              & 35.00               & 40.00            & 36.67           & 35.00            & 40.00        \\

\arrayrulecolor{black}\thicktablehline

\textbf{Micro Average}                    & \textbf{78.03}     & \textbf{88.84}         & \textbf{69.60}     & \textbf{76.97}    & \textbf{87.91}       & \textbf{68.48}    & \textbf{76.78}   & \textbf{87.51}      & \textbf{68.42}  \\

\hline

\end{tabular}

\label{table:nlp:performance}
\end{table*}
